OSOM: A simultaneously optimal algorithm for multi-armed and linear contextual bandits

We consider the stochastic linear (multi-armed) contextual bandit problem with the possibility of hidden simple multi-armed bandit structure in which the rewards are independent of the contextual information. Algorithms that are designed solely for one of the regimes are known to be sub-optimal for the alternate regime. We design a single computationally efficient algorithm that simultaneously obtains problem-dependent optimal regret rates in the simple multi-armed bandit regime and minimax optimal regret rates in the linear contextual bandit regime, without knowing a priori which of the two models generates the rewards. These results are proved under the condition of stochasticity of contextual information over multiple rounds. Our results should be viewed as a step towards principled data-dependent policy class selection for contextual bandits.

==> lowerbound.tex <==
\section{Problem-dependent, Asymptotic Lower Bound}

Theorem~\ref{thm:mainregretbound} gives us a positive result in terms of minimax-optimality: we simultaneously obtain the \textit{instance-optimal} rate for the simple model ($\mathcal{O}(\log n)$ when we substitute $\delta = \frac{1}{n}$ in the high-probability bound), and the \textit{minimax-optimal} rate for the complex model ($\widetilde{\mathcal{O}}((\sqrt{d} + \sqrt{K})\sqrt{n})$). 
We critically made the assumption for our result that the contexts need to arrive from an iid distribution.
We show below that this assumption is essentially necessarily in the \textit{problem-dependent} sense. 
%In the context of the positive, minimax-optimal result of Theorem~\ref{thm:mainregretbound}, it is reasonable to ask whether we can obtain even stronger \textit{problem-dependent rates}; that is, the $\mathcal{O}(\log n)$ rates for the simple model and the $\mathcal{O}(d \log n)$ rate for the complex model\footnote{the authors of OFUL~\cite{abbasi2011improved} obtain a problem-dependent upper bound $\mathcal{O}\left( \frac{1}{\Delta} \left( \log^2 n + d \log n \right) \right)$ where $\Delta := \min_{1 \leq t \leq n} \Delta_t$ and $\Delta_t$ is the expected gap between the reward of the best arm and the second best arm in round $t$.}.
%Note that the analysis we have presented does not help with this goal, as we have allowed for fluctuations on the order of $\sqrt{n}$.
We consider the special case of $K = 2$ arms and show that, for a fixed $d > 0$ and an engineered set of contexts, to be able to retain a logarithmic rate \textit{in the number of rounds $n$} for complex model instances, we need to pay the model complexity factor in the simple model regime as well.
Before stating the main result of this section, we introduce some additional probabilistic notation.

\begin{definition}
Let $w(\cdot)$ be the probability density function of the identical, independent, zero-mean noise $\{\eta_{i,t}\}_{i=1}^K$ such that $\int_{-\infty}^{\infty} |x| w(x) dx < \infty$\footnote{This is automatically implied from sub-Gaussianity; see~\cite[Chap.2,]{}.}.
Then, we define the PDF of random variable $R = \mu_k + \eta$ by $r_k(\cdot;w)$.
\textcolor{red}{\textbf{It should be implicit that the distributions are absolutely continuous, but make sure to specify this.}}
We denote as shorthand
\begin{align}\label{eq:kldefinition}
    D(\mu_k, \mu_{k'};w) := D_{KL}(r_k(\cdot;w) || r_{k'}(\cdot;w))
\end{align}

where $D_{KL}(\cdot || \cdot)$ denotes the KL divergence between two distributions.
\end{definition}

\begin{definition}
For a given noise pdf $w(\cdot)$, we parameterize simple model (SM) instances by the means $s = (\mu_1, \mu_2) \in [-1,1] \times [-1,1]$.
Further, we parameterize complex model (CM) instances by two quantities:
\begin{enumerate}
    \item The means and parameter vector $(\mu_1,\mu_2, \theta^*)$ where $\theta^* \in \mathbb{B}_2^d(1)$.
    \item The context sequence $\{\{\alpha_{i,t}\}_{t\geq 1}\}_{i=1}^K$. 
\end{enumerate}
\end{definition}

Note that we have included the context sequence itself as a part of the definition of the complex model instance. We are now ready to state our main result below.

\begin{theorem}\label{thm:lowerbound}
For every simple instance $s = (\mu_1, \mu_2)$, there exists a complex instance $c = (\mu_1,\mu_2,\theta^*; \{\{\alpha_{i,t}\}_{t\geq 1}\}_{i=1}^K)$ such that:
\begin{align*}
    R_n^c &= \mathcal{O}(n^a) \text{ for all $a > 0$ and for all $c \in \mathcal{C}$} \\
    \implies {\lim \inf}_{n \to \infty} \frac{R_n^s}{\log \left(n/d\right)} &\geq \frac{(d/2 + 1) \cdot \Delta}{D(\mu_2,\mu_1;w)} 
\end{align*}
where $D(\cdot,\cdot;w)$ is as defined in Equation~\eqref{eq:kldefinition}.
\end{theorem}

Note that $d \log \left(n/d\right) > \log n$ by a substantial amount when $n >> d >> 1$, which is typically the regime of interest\footnote{If $d << n$ for instance, it is typically not useful to exploit the linear structure and an expert-based algorithm gives the optimal guarantee.}.
Theorem~\ref{thm:lowerbound} implies that we need to pay an extra model complexity factor even in simple instances to be able to distinguish all complex instances to the extent required for logarithmic regret rates with the horizon.
Like the Lai-Robbins lower bound, we proceed by reducing the composite testing problem to a set of simple (multiple) hypotheses.

\begin{Proof}
Consider simple instance $s = (\mu_1, \mu_2)$.
We define the following context instance $\{X_{1,t}, X_{2,t}\}_{t \geq 1}$:
\begin{align*}
    X_{1,t} &= \hat{e}_1 \\
    X_{2,t} &= \hat{e}_{t (\mod d) + 1}
\end{align*}

where $\hat{e}_j, j \in \{1,2,\ldots, d\}$ represents the standard basis vector in $\mathbb{R}^d$.
Next, we define our set of complex instances below.

\begin{definition}\label{def:complexconstructions}
For a subset $S \subset [d]: |S| = d/2$, we define special complex instance 
\begin{align*}
c(S, \epsilon;(\mu_1, \mu_2)) &:= \theta^*(S, \epsilon;(\mu_1,\mu_s)) \text{ where } \\
    \theta^*(S;(\mu_1,\mu_2))_j &:= \begin{cases}
    \mu_2 \text{ if } j \notin S \\
    \mu_1 + \epsilon \text{ if } j \in S .
    \end{cases}
\end{align*}

Corresponding to simple instance $s = (\mu_1,\mu_2)$, we will consider the class of special context instances $\mathcal{C} := \{c(S, \epsilon;s): S \subset [d], |S| = d/2\}$.
\end{definition}

The intuition behind the constructions in Definition~\ref{def:complexconstructions} is clear: the contexts for arm $1$ give no information about $\theta^*$.
Even if we were given oracle information that arm $1$ is better than arm $2$ under the simple model, we are forced to explore arm $2$ some minimum number of times to learn which environment we are in.
In fact, we are forced to explore arm $2$ in a very specific way, as we describe below.

\begin{lemma}\label{lem:samplinglowerbound}
We denote $\mathbb{E}_s$ to be the expectation under the stochastic process induced by instance $c$.
Further, (this is a definition very specific to the context choice outlined above) denote $T_2(n;j) := \sum_{t=1}^n \mathbb{I}[I_t = 2; t \mod d + 1 = j]$ for every $j \in [d]$.

Then, there exists a set $S' \in [d]: |S'| > d/2$ such that
\begin{subequations}
\begin{align}
    \mathbb{E}_c[R_n^c] &= \mathcal{O}(n^a) \text{ for all $a > 0$ and for all $c \in \mathcal{C}$} \label{eq:complexcondition} \\
    \implies {\lim \inf}_{n \to \infty} \frac{\mathbb{E}_s[T_2(n;j)]}{\log \left(n/d\right)} &\geq \frac{1}{D_{KL}(\mu_2 || \mu_1)} \text{ for all } j \in S' . \label{eq:samplinglowerbound}
\end{align}
\end{subequations}

\end{lemma}

Clearly, the proof of Theorem~\ref{thm:lowerbound} follows easily from Lemma~\ref{lem:samplinglowerbound}, because
\begin{align*}
    {\lim \inf}_{n \to \infty} \frac{\mathbb{E}_s[T_2(n)]}{\log \left(n/d\right)} &= {\lim \inf}_{n \to \infty} \frac{\sum_{j=1}^d \mathbb{E}_s[T_2(n;j)]}{\log \left(n/d\right)} \\
    &\geq {\lim \inf}_{n \to \infty} \frac{\sum_{j \in S'} \mathbb{E}_s[T_2(n;j)]}{\log \left(n/d\right)} \\
    &\geq \sum_{j \in S'} {\lim \inf}_{n \to \infty} \frac{\mathbb{E}_s[T_2(n;j)}{\log \left(n/d\right)} ,
\end{align*}

where the first inequality follows because of pointwise non-negativity of $T_2(n;j)$ for all $j$, and the second inequality follows because we take the inf inside of the individual sums.
Then, we have $\mathbb{E}_s[R_n^s] = \Delta \mathbb{E}_s[T_2(n)]$ and the original statement of Theorem~\ref{thm:lowerbound} easily follows.
Thus, we devote the rest of the proof to proving Lemma~\ref{lem:samplinglowerbound}.

\begin{Proof}
Observe that for a given complex instance $c(S,\epsilon;s)$, we have 
\begin{align*}
    \mathbb{E}_c[R_n^c] &= \sum_{j \in S} \epsilon \cdot \mathbb{E}_c[T_1(n;j)] + \sum_{j \notin S} \Delta \mathbb{E}_c[T_2(n;j)] .
\end{align*}

Now, let condition~\eqref{eq:samplinglowerbound} be violated.
Then, there exists a set $S^*$ of size $d/2$ such that 
\begin{align}\label{eq:toofewsamples}
    {\lim \inf}_{n \to \infty} \frac{\mathbb{E}_s[T_2(n;j)]}{\log \left(n/d\right)} < \frac{1}{D_{KL}(\mu_2 || \mu_1)} \text{ for all } j \in S^* .
\end{align}

\note{This is the set $S^*$ of contexts for which the second arm is actually better than the first arm, and sampling the first arm is suboptimal.}

We consider the particular complex instance $c(S^*, \epsilon; s)$.
We will use a change-of-measure argument to claim that under the condition of Equation~\eqref{eq:toofewsamples}, simple instance $s$ and complex instance $c(S^*, \epsilon;s)$ cannot be sufficiently distinguished.
Effectively, we'll show that for all $j \in S^*$,
\begin{align*}
    \mathbb{E}_c[T_2(n;j)] &\leq () \mathbb{E}_s[T_2(n;j)] \\
    &< () \frac{\log \left(n/d\right)}{D_{KL}(\mu_2 ||\mu_1)} \text{ for all } j \in S^*. 
\end{align*}

\note{To do: write completely rigorously using Bubeck Cesa-Bianchi Chapter $2$ writing style.}
This implies that there exists some $a > 0$ for which
\begin{align*}
    \mathbb{E}_d[T_1(n;j)] &= \Omega(\left(\frac{n}{d}\right)^a) \text{ for all } j \in S^*\\
    \implies \mathbb{E}_c[R_n^c] = \epsilon \cdot \Omega(d \cdot \left(\frac{n}{d}\right)^a) 
\end{align*}

and this particular complex instance would suffer more than logarithmic regret asymptotically.
This can only be avoided if condition~\eqref{eq:samplinglowerbound} is in fact satisfied. 
This completes the proof of Lemma~\ref{lem:samplinglowerbound}.
\end{Proof}
\end{Proof}

